ILIAS: Instance-Level Image retrieval At Scale

This work introduces ILIAS, a new test dataset for Instance-Level Image retrieval At Scale. It is designed to evaluate the ability of current and future foundation models and retrieval techniques to recognize particular objects. The key benefits over existing datasets include large scale, domain diversity, accurate ground truth, and a performance that is far from saturated. ILIAS includes query and positive images for 1,000 object instances, manually collected to capture challenging conditions and diverse domains. Large-scale retrieval is conducted against 100 million distractor images from YFCC100M. To avoid false negatives without extra annotation effort, we include only query objects confirmed to have emerged after 2014, i.e. the compilation date of YFCC100M. An extensive benchmarking is performed with the following observations: i) models fine-tuned on specific domains, such as landmarks or products, excel in that domain but fail on ILIAS ii) learning a linear adaptation layer using multi-domain class supervision results in performance improvements, especially for vision-language models iii) local descriptors in retrieval re-ranking are still a key ingredient, especially in the presence of severe background clutter iv) the text-to-image performance of the vision-language foundation models is surprisingly close to the corresponding image-to-image case. website: https://vrg.fel.cvut.cz/ilias/

==> data/instre_gld_sop.tex <==
\pgfplotstableread{
model	INSTRE	GLDv2	SOP ILIAS show
alexnet.tv_in1k	26.81	2.36	31.53	1.5	0
vgg16.tv_in1k	33.85	4.11	32.47	2.3	0
resnet50.tv_in1k	24.45	4.41	36.23	1.7	0
resnet101.tv_in1k	27.20	4.42	36.37	1.9	0
densenet169.tv_in1k	27.23	4.95	37.28	2.4	0
inception_v4.tf_in1k	24.52	3.44	24.84	1.1	0
nasnetalarge.tf_in1k	27.32	3.28	23.50	1	0
tf_efficientnet_b4.ns_jft_in1k	38.44	5.38	31.11	2.6	0
vit_base_patch16_224.augreg_in1k	25.17	2.49	31.78	1	0
vit_base_patch16_224.augreg_in21k	44.73	7.24	45.78	3	0
vit_large_patch16_224.augreg_in21k	47.95	9.69	50.18	4.6	0
vit_large_patch16_224.augreg_in21k_ft_in1k	47.42	8.98	45.12	3.6	0
vit_large_patch16_384.augreg_in21k_ft_in1k	54.99	11.10	46.00	5.3	0
dino_resnet50	27.18	5.43	42.24	2.9	0
dino_vitb16	36.55	7.00	38.78	3.7	0
swav	18.81	4.93	39.67	1.7	0
moco_v3_resnet50	27.50	6.76	36.20	2.6	0
moco_v3_vit	25.62	4.89	40.99	1.9	0
RN50.openai	49.50	8.45	42.69	3.2	1
vit_base_patch16_clip_224.openai	59.97	10.16	35.23	4.2	1
vit_large_patch14_clip_224.openai	67.65	12.56	38.08	7	1
vit_large_patch14_clip_336.openai	72.96	14.33	39.41	9.4	1
vit_large_patch14_clip_224.laion2b	69.84	16.42	50.68	9.4	1
deit3_base_patch16_224.fb_in1k	30.17	4.28	28.13	1.2	0
deit3_large_patch16_224.fb_in1k	32.04	4.23	29.05	1.5	0
convnext_base.fb_in1k	35.32	3.90	32.64	2	0
convnext_large.fb_in1k	36.61	3.86	32.33	2.2	0
convnext_base.fb_in22k	54.00	11.82	46.75	6.4	0
convnext_large.fb_in22k	53.98	10.47	48.30	6.6	0
convnext_base.clip_laion2b_augreg	65.03	13.53	50.41	7.9	1
convnext_large_mlp.clip_laion2b_ft_soup_320	68.67	16.79	54.26	9.6	1
cvnet_resnet50	29.82	29.72	46.04	2.9	3
cvnet_resnet101	30.90	32.17	46.43	3	3
eva02_base_patch14_224.mim_in22k	38.76	11.05	40.43	2.1	0
eva02_large_patch14_224.mim_in22k	39.38	10.36	36.90	1.5	0
eva02_large_patch14_224.mim_m38m	50.76	17.24	46.05	4.7	0
eva02_base_patch16_clip_224.merged2b	61.22	11.96	45.16	5.9	1
eva02_large_patch14_clip_336.merged2b	71.67	19.00	50.03	10.9	1
superglobal_resnet50	34.06	29.58	43.95	3.4	3
superglobal_resnet101	36.76	31.87	44.35	3.4	3
recall_512-resnet50	23.85	1.13	64.55	1.6	4
recall_512-vit_base_patch16_224_in21k	54.02	4.02	79.09	5	4
unicom_vit_base_patch16_224	70.59	20.20	51.43	11	5
unicom_vit_large_patch14_224	80.94	21.83	53.52	13.8	5
unicom_vit_large_patch14_336	80.08	23.32	56.34	13.9	5
unicom_vit_base_patch16_sop	56.26	15.78	78.90	9.1 4
unicom_vit_base_patch16_gldv2	34.08	36.62	45.19 3	3
dinov2_vitb14	55.39	26.27	32.87	11.5	2
dinov2_vitl14	61.01	29.86	33.83	15.3	2
dino_vit16_patch16_224_sop	41.56	3.55	70.87	3.3    4
vit_base_patch16_siglip_224.webli	74.17	11.95	48.94	11.2	1
vit_base_patch16_siglip_256.webli	73.91	11.03	48.33	11.5	1
vit_base_patch16_siglip_384.webli	80.35	13.92	52.01	15.6	1
vit_base_patch16_siglip_512.webli	82.65	15.06	51.16	16.6	1
vit_large_patch16_siglip_256.webli	78.81	15.65	52.87	15.2	1
vit_large_patch16_siglip_384.webli	82.85	18.26	56.38	19.6	1
vit_base_patch16_clip_224.metaclip_2pt5b	62.09	10.46	48.75	6.6	1
vit_large_patch14_clip_224.metaclip_2pt5b	68.14	15.96	48.53	11.7	1
dinov2_vitb14_reg	56.02	27.66	32.32	9.4	2
dinov2_vitl14_reg	63.27	31.23	33.29	9.4	2
udon_64-vit_base_patch16_clip_224.openai	58.82	22.25	68.10	5.9	5
uscrr_64-vit_base_patch16_clip_224.openai	53.58	16.59	65.15	3.8	5
udon_64-vit_base_patch16_224.augreg_in21k_ft_in1k	45.68	19.56	64.94	5.5 5
unic_l	65.73	20.22	40.20	8.9	5
vit_base_patch16_siglip_384.v2_webli	82.35	14.76	53.84	15	1
vit_base_patch16_siglip_512.v2_webli	83.78	15.71	52.84	15.4	1
vit_large_patch16_siglip_384.v2_webli	82.63	17.69	60.00	19.9	1
vit_large_patch16_siglip_512.v2_webli	83.19	18.28	58.51	20.8	1
}{\instregldsop}

==> data/instre_gld_sop_adapt.tex <==
\pgfplotstableread{
model	INSTRE	GLDv2	SOP ILIAS show
alexnet.tv_in1k	27.67	2.47	32.13	1.3	0
vgg16.tv_in1k	32.89	4.30	32.27	1.6	0
resnet50.tv_in1k	29.60	5.45	35.31	1.8	0
resnet101.tv_in1k	31.24	5.21	35.84	1.8	0
densenet169.tv_in1k	29.72	6.35	36.15	2	0
inception_v4.tf_in1k	25.13	4.75	25.48	1	0
nasnetalarge.tf_in1k	27.23	4.70	24.25	1	0
tf_efficientnet_b4.ns_jft_in1k	41.84	8.09	32.96	2.9	0
vit_base_patch16_224.augreg_in1k	28.27	4.87	34.69	1.3	0
vit_base_patch16_224.augreg_in21k	50.80	12.45	47.62	4.4	0
vit_large_patch16_224.augreg_in21k	50.54	14.07	49.36	5.3	0
vit_large_patch16_224.augreg_in21k_ft_in1k	52.35	14.07	46.72	4.7	0
vit_large_patch16_384.augreg_in21k_ft_in1k	59.05	15.94	47.77	6.4	0
dino_resnet50	34.70	9.97	44.00	2.9	0
dino_vitb16	42.38	10.58	42.12	4.8	0
swav	26.27	10.01	41.23	2.1	0
moco_v3_resnet50	32.82	9.71	36.39	2.6	0
moco_v3_vit	32.63	8.32	41.29	2.3	0
RN50.openai	68.25	13.66	47.71	6	1
vit_base_patch16_clip_224.openai	77.79	15.50	40.64	7.9	1
vit_large_patch14_clip_224.openai	81.77	20.80	42.37	11.9	1
vit_large_patch14_clip_336.openai	85.52	22.13	43.79	15.2	1
vit_large_patch14_clip_224.laion2b	80.91	22.03	54.98	13.7	1
deit3_base_patch16_224.fb_in1k	35.01	7.71	31.85	1.8	0
deit3_large_patch16_224.fb_in1k	39.58	8.42	34.21	2.4	0
convnext_base.fb_in1k	37.58	7.93	38.43	2.7	0
convnext_large.fb_in1k	38.75	8.40	38.96	2.9	0
convnext_base.fb_in22k	55.66	15.76	48.04	7.6	0
convnext_large.fb_in22k	52.96	15.94	49.74	6.9	0
convnext_base.clip_laion2b_augreg	77.91	19.12	54.80	14	1
convnext_large_mlp.clip_laion2b_ft_soup_320	83.03	24.34	58.93	18.3	1
cvnet_resnet50	29.89	29.18	44.25	2.6	3
cvnet_resnet101	31.89	31.53	44.88	3.1	3
eva02_base_patch14_224.mim_in22k	49.51	15.44	44.27	3.2	0
eva02_large_patch14_224.mim_in22k	51.73	14.66	41.17	2.7	0
eva02_large_patch14_224.mim_m38m	63.23	22.67	50.06	6.1	0
eva02_base_patch16_clip_224.merged2b	73.85	17.33	50.36	8.7	1
eva02_large_patch14_clip_336.merged2b	84.02	26.82	55.79	16	1
superglobal_resnet50	31.68	28.74	41.39	2.8	3
superglobal_resnet101	34.67	30.73	41.38	3.2	3
recall_512-resnet50	36.51	4.44	59.61	2.1	4
recall_512-vit_base_patch16_224_in21k	54.76	8.68	74.42	5.3	4
unicom_vit_base_patch16_224	69.15	20.56	51.47	11.1	5
unicom_vit_large_patch14_224	80.45	23.34	52.81	13.8	5
unicom_vit_large_patch14_336	79.74	24.55	55.76	14.6	5
unicom_vit_base_patch16_sop	60.35	18.72	74.46	9.9	4
unicom_vit_base_patch16_gldv2	35.50	36.36	45.67	3.3	3
dinov2_vitb14	56.02	27.32	35.23	12.1	2
dinov2_vitl14	60.30	30.63	35.65	15.3	2
dino_vit16_patch16_224_sop	45.25	6.15	66.29	3.6	4
vit_base_patch16_siglip_224.webli	83.04	16.90	54.27	15.7	1
vit_base_patch16_siglip_256.webli	83.13	17.10	53.72	16.7	1
vit_base_patch16_siglip_384.webli	87.97	19.22	57.21	21.5	1
vit_base_patch16_siglip_512.webli	89.26	20.80	57.14	23	1
vit_large_patch16_siglip_256.webli	86.74	21.60	58.97	21.8	1
vit_large_patch16_siglip_384.webli	90.35	24.33	62.30	28.9	1
vit_base_patch16_clip_224.metaclip_2pt5b	77.29	17.02	51.71	9.4	1
vit_large_patch14_clip_224.metaclip_2pt5b	82.26	22.44	53.29	16.9	1
dinov2_vitb14_reg	56.77	28.95	35.47	10.7	2
dinov2_vitl14_reg	63.24	32.37	35.60	13.6	2
udon_64-vit_base_patch16_clip_224.openai	59.42	22.78	68.79	6.7	5
uscrr_64-vit_base_patch16_clip_224.openai	55.40	18.26	65.69	4.3	5
udon_64-vit_base_patch16_224.augreg_in21k_ft_in1k	44.99	20.44	66.34	5.3	5
unic_l	73.24	23.49	46.87	11.7	5
vit_base_patch16_siglip_384.v2_webli	90.01		20.68		60.37			22.6	1
vit_base_patch16_siglip_512.v2_webli	90.97		21.75		59.86			23.5	1
vit_large_patch16_siglip_384.v2_webli	91.48		26.21		65.86			30.3	1
vit_large_patch16_siglip_512.v2_webli	92.03		26.59		65.21			31.3	1
}{\instregldsop}

==> fig/fig_heatmaps_scale.tex <==
\vfill
\centering
\scalebox{0.97}{
\begin{tabular}{cc}
    \hspace{-25pt}
    \begin{subfigure}{0.22\textwidth}
        \centering
        \input{fig/fig_heatmap_db_rank_vs_clutter}
        \vspace{-2.7pt}
        \caption{\label{fig:heatmap_db_rank_vs_clutter}}
    \end{subfigure}
    &
    \hspace{-41pt}
    \begin{subfigure}{0.22\textwidth}
        \centering
        \input{fig/fig_heatmap_db_rank_vs_scale}
        \vspace{-3pt}
        \caption{\label{fig:heatmap_db_rank_vs_scale}}
    \end{subfigure}
\end{tabular}
}
